Subspace Recycling-based Regularization Methods

Subspace recycling techniques have been used quite successfully for the acceleration of iterative methods for solving large-scale linear systems. These methods often work by augmenting a solution subspace generated iteratively by a known algorithm with a fixed subspace of vectors which are ``useful'' for solving the problem. Often, this has the effect of inducing a projected version of the original linear system to which the known iterative method is then applied, and this projection can act as a deflation preconditioner, accelerating convergence. Most often, these methods have been applied for the solution of well-posed problems. However, they have also begun to be considered for the solution of ill-posed problems. In this paper, we consider subspace augmentation-type iterative schemes applied to linear ill-posed problems in a continuous Hilbert space setting, based on a recently developed framework describing these methods. We show that under suitable assumptions, a recycling method satisfies the formal definition of a regularization, as long as the underlying scheme is itself a regularization. We then develop an augmented subspace version of the gradient descent method and demonstrate its effectiveness, both on an academic Gaussian blur model and on problems arising from the adaptive optics community for the resolution of large sky images by ground-based extremely large telescopes.

==> non-linear-landweber.tex <==
%!TEX root = aug-simple-landweber.tex
\section{Augmenting non-linear Landweber iterations}
All that we have presented up to now has been for linear well- and ill-posed problems.  However, in this section, we justify the 
utility in using this augmentation technique for non-linear problems, particularly the nonlinear Landweber iteration.  

Consider now the nonlinear equation
\be\label{eqn.Fxy}
	F(x)  =y\mwith F:\CD(F)\subset\CX\rightarrow\CY\mbox{ is nonlinear},
\ee
such that $F$ is continuous and weakly sequentially closed (EHN condition).  In Algorithm \ref{alg.nonlinear-grad-desc}, we remind the reader of the non-linear
gradient descent method.  Here, we do not specify what $\alpha_{i}$ is; it is simply some parameter determining how far we go along the gradient direction at step $i$.
Not that $F'(x_{i})$ denotes the Frechet derivative at $x_{i}$.
\balgte[H]\label{alg.nonlinear-grad-desc}
\caption{Non-linear gradient descent method}
Set $r_{0} = y - F(x_{0})$\\
\For{i=0,1,2,\ldots}{
	$x_{i+1} = x_{i} + \alpha_{i}F'(x_{i})^{\ast}r_{i}$\\
	$r_{i+1} = y - F(x_{i+1})$
}
\ealgte
Observe that one can interpret Algorithm \ref{alg.nonlinear-grad-desc} as taking a step in the gradient direction of the normal equations
for the local linearization of the problem 
\be\label{eqn.Frechet-linear}
	F'(x_{i}) t_{i} = r_{i}
\ee
generated by the Frechet derivative at the current iterate.  Consider the case when we choose $\alpha_{i}$ at each iteration such that
we are taking the steepest descent step with respect to \cref{eqn.Frechet-linear} at $x_{i}$. 
 Consider that in the linear case \cref{illposedeq}, this iteration could be modified
to become conjugate gradients applied to the normal equations by simply enforcing the each new gradient direction is orthogonal in the $T^{\ast}T$-norm
to all previous directions. Furthermore, we know that this reduces to orthogonalizing against the two most recent directions, as each new gradient 
direction is automatically $T^{\ast}T$-orthogonal to all other previous. 
For non-linear gradient (steepest) descent, none of this holds.  There is not even a fixed operator norm
for which to consider this scenario.  However, one can still mimic the construction of a conjugate gradient type direction by saving the gradient directions 
at some or all previous iterations and
storing them in $\CU$, then applying one iteration of augmented gradient descent (Landweber) to \cref{eqn.Frechet-linear}.  
However, one must modify a few steps to 
accommodate the changing Frechet derivative at every iteration.  

Following from how Algorithm \ref{alg.aug-Landweber} was derived, we propose that one similarly 
apply the same linear projection to the nonlinear
equation, yielding
\be\label{eqn.proj-nonlinear}
	\prn{I_{\CY} - Q}F(x)  =\prn{I_{\CY} - Q}y.
\ee
We then follow the same procedure, namely that we apply iterations of the non-linear Landweber iteration to this projected non-linear equation and then
apply the same projectors used in Algorithms \ref{alg.aug-steepest-descent} and \ref{alg.aug-Landweber} to recover the correction from $\CU$.  To do this, we first
need to calculate the Frechet derivative of $\widetilde{F}$ defined by $\widetilde{F}(x) = \prn{I_{\CY} - Q}F(x)$.  Under some assumptions [NEED TO CHECK
ON THESE], the usual chain rule holds for the Frechet derivative.  Furthermore, we note that since $Q$ is a linear operator, it is its own Frechet
derivative which is constant on the whole domain.  Thus, we compute the Frechet derivative of a nonlinear operator of the form $P\circ F$ where $P$ is the linear
projector.
Thus, we have
\be\nn
	\prn{P\circ F}'(x) = P'(F(x))\circ F'(x) = P\circ F'(x),
\ee
and $\widetilde{F}'(x) = \prn{I_{\CY} - Q}F'(x)$.

The second issue is, how do we obtain subspace $\CC$?  Because $F$ is nonlinear, the choice $\CC=F(\CU)$ does not produce any kind of optimal projection.
A better choice is to calculate at every iteration $\CC_{i} = F'(x_{i})\CU$.  Then we let $\vek Q_{i} = I_{\CY} - \vek C_{i}\vek C_{i}^{\ast}$ 
be the orthogonal projector onto $\CC_{i}$, and 
we let $\vek P_{\CU,i}^{(MR)}$ be the corresponding $F'(x_{i})^{\ast}F'(x_{i})$-orthogonal projector onto $\CU$.
Thus we propose as a candidate for an augmented non-linear Landweber method, to apply the non-linear Landweber method (Algorithm \ref{alg.nonlinear-grad-desc}) 
to the projected non-linear problem \cref{eqn.proj-nonlinear}.  At iteration $i$, we perform the same projections as in augmented linear Landweber
to get the correction $s_{i}\in\CU$.  Thus we propose Algorithm \ref{alg.aug-nonlinear-landweber}.


\balgte\label{alg.aug-nonlinear-landweber}
\caption{Augmented linear Landweber for the normal equations}
Given: $\alpha\in\R$ and $\vek U\in\R^{n\times k}$ representing $\CU$\\
Set $r_{0} = y - F(x_{0})$\\
Compute {\tt QR}-factorization $F'(x_{0})\vek U = \vek C\vek R$\\
$\vek U\leftarrow \vek U\vek R^{-1}$\\
$\vek u^{(1)} \leftarrow \prn{r_{0},\vek C}_{\CY}$\\
$x \leftarrow x_{0} + \vek U\vek u^{(1)}  $\\
$r  \leftarrow y - F(x)  $\\
\While{STOPPING-CRITERIA}{
	Compute {\tt QR}-factorization $F'(x)\vek U = \vek C\vek R$\\
	$\vek U\leftarrow \vek U\vek R^{-1}$\\
	$\widehat{\vek w}\leftarrow = \prn{F'(x)F'(x)^{\ast}\prn{I_{\CY} - Q}r,\vek C}_{\CY}$\\
	$x\leftarrow x + \alpha F'(x)^{\ast}\prn{I_{\CY} - Q}r - \alpha \vek U\widehat{\vek w}$\\
	$r\leftarrow y - F(x)$
}
Compute {\tt QR}-factorization $F'(x)\vek U = \vek C\vek R$\\
$\vek U\leftarrow \vek U\vek R^{-1}$\\
$\vek u^{(1)} \leftarrow \prn{r,\vek C}_{\CY}$\\
$x \leftarrow x + \vek U\vek u^{(1)}  $\\
$r  \leftarrow y - F(x)  $
\ealgte

Consider that the proposed method can be interpreted at each iteration as taking one step of the augmented linear Landweber method for
the linear operator $F'(x_{i})$ using the $\CC_{i}$ generated using the Frechet derivative at this point.
